Shuffle Gaussian Mechanism for Differential Privacy

We study Gaussian mechanism in the shuffle model of differential privacy (DP). Particularly, we characterize the mechanism's R\'enyi differential privacy (RDP), showing that it is of the form: $$ \epsilon(\lambda) \leq \frac{1}{\lambda-1}\log\left(\frac{e^{-\lambda/2\sigma^2}}{n^\lambda} \sum_{\substack{k_1+\dotsc+k_n = \lambda; \\k_1,\dotsc,k_n\geq 0}}\binom{\lambda}{k_1,\dotsc,k_n}e^{\sum_{i=1}^nk_i^2/2\sigma^2}\right) $$ We further prove that the RDP is strictly upper-bounded by the Gaussian RDP without shuffling. The shuffle Gaussian RDP is advantageous in composing multiple DP mechanisms, where we demonstrate its improvement over the state-of-the-art approximate DP composition theorems in privacy guarantees of the shuffle model. Moreover, we extend our study to the subsampled shuffle mechanism and the recently proposed shuffled check-in mechanism, which are protocols geared towards distributed/federated learning. Finally, an empirical study of these mechanisms is given to demonstrate the efficacy of employing shuffle Gaussian mechanism under the distributed learning framework to guarantee rigorous user privacy.

==> app_exp.tex <==
\section{Experimental Details}
\label{app:exp}
\noindent \textbf{Network architecture.}
The neural network we use in the experiments presented in Section \ref{sec:numerics} is as in Table \ref{tab:nn}.
\begin{table}[]
 \caption{Neural network architecture used in our experiment.}
    \label{tab:nn}
    \centering
    \begin{tabular}{c|c}
    \toprule
        Layer & Parameters  \\
                        \midrule
        Convolution & 16 filters of $8\times8$ , strides 2 \\
        Max-pooling & $2\times2$ \\
        Convolution & 32 filters of $4\times4$, strides 2\\
        Max-pooling & $2\times2$ \\
        Linear & 32 units \\
        Softmax & 10 units \\
        \bottomrule
    \end{tabular}
\end{table}

\noindent \textbf{Baseline for privacy accounting of shuffled check-in with generic LDP mechanism.}
We here describe in more detail our method of shuffled check-in with generic LDP mechanism without using Theorem \ref{th:main}.

Our shuffled check-in protocol has an issue that cannot be dealt with using standard subsampling/shuffling techniques: the number of clients checking in is a variable, following a probability distribution equal to those followed by $k$ in Equation \ref{eq:main}.

To resolve this, we devise the following method.
Given $0\leq \delta'\leq 1$, we first find $l$ such that, $\mathbb{P}[k\leq l]= 1-\delta'$ for $k$ and the corresponding binomial probability distribution defined in Equation \ref{eq:main}.
Fixing the number of clients to be $l$, we the use the following to \textit{conservatively} bound the approximate DP of subsampled shuffling:
\begin{itemize}
\item No privacy amplification occurs ($\eps=\eps_0$) due to shuffling (see Footnote \ref{fn:shuff}).
\item Privacy amplification by subsampling is accounted for by assuming conservatively that $l$ clients are sampled. 
More precisely, let $\gamma' = l/n$, privacy amplification by subsampling leads to $\eps_1 = \log (1+ \gamma' (e^{\eps_0}-1))$ and $\delta_1 = \gamma'\delta_0$ \cite{balle2018privacy}.
\end{itemize}
Consequently, the approximate DP of shuffled check-in for a single round is $(\eps_1, \delta_1 + \delta')$ by absorbing $\delta'$ to the final DP.
To compose the mechanism, we convert the approximate DP to RDP as done in Section \ref{subsec:gen} and use Lemma \ref{lm:rdpcompose}. \footnote{We find that composition using the strong composition theorem \cite{kairouz2015composition} leads to a much looser privacy accounting.}

\noindent \textbf{Federated DP-SGD.}
Given $\eps_0$, we fix $\delta_0=1/n^{1.5}$ to calculate the noise multiplier $z$ of the Gaussian mechanism, which adds Gaussian noise, $N(0,z^2C^2I)$ to the gradient \cite{abadi2016deep}.

In Figure \ref{fig:feddpsgd}, we show the accuracy-round curve of our Federated DP-SGD experiment with the following parameters:
$\eps_0=8$, $n= 10^7$ (by bootstrapping from the train dataset), $\gamma = 10^{-4}$, clipping size $C=0.05$.
It should be noted that the average number of clients checking in is 1,000, around the same order as the ones used in the settings given in Section \ref{sec:numerics}.
It can then be seen that the accuracy can reach the optimal $90\%$, and converges faster with a larger $\eps_0$, noting that $n$ mainly affects the final $\eps$, not the convergence. 
Note also that we have not evaluated the accuracy with respect to all ranges of $\eps$ in this experiment as it is computationally too expensive.
\begin{figure}
  \begin{center}
    \includegraphics[width=0.6\textwidth]{nips/figs/n_10_7_delta0_1_5_eps0_8_gamma_0_0001_times_10000.png}
  \end{center}
  \caption{Federated DP-SGD.}
      \label{fig:feddpsgd}
\end{figure}

